Lite-PoT: Practical Powers-of-Tau Setup Ceremony

Zero-Knowledge Succinct Non-Interactive Argument of Knowledge (zk-SNARK) schemes have gained significant adoption in privacy-preserving applications, decentralized systems (e.g., blockchain), and verifiable computation due to their efficiency. However, the most efficient zk-SNARKs often rely on a one-time trusted setup to generate a public parameter, often known as the ``Powers of Tau" (PoT) string. The leakage of the secret parameter, $\tau$, in the string would allow attackers to generate false proofs, compromising the soundness of all zk-SNARK systems built on it. Prior proposals for decentralized setup ceremonies have utilized blockchain-based smart contracts to allow any party to contribute randomness to $\tau$ while also preventing censorship of contributions. For a PoT string of $d$-degree generated by the randomness of $m$ contributors, these solutions required a total of $O(md)$ on-chain operations (i.e., in terms of both storage and cryptographic operations). These operations primarily consisted of costly group operations, particularly scalar multiplication on pairing curves, which discouraged participation and limited the impact of decentralization In this work, we present Lite-PoT, which includes two key protocols designed to reduce participation costs: \emph{(i)} a fraud-proof protocol to reduce the number of expensive on-chain cryptographic group operations to $O(1)$ per contributor. Our experimental results show that (with one transaction per update) our protocol enables decentralized ceremonies for PoT strings up to a $2^{15}$ degree, an $\approx 16x$ improvement over existing on-chain solutions; \emph{(ii)} a proof aggregation technique that batches $m$ randomness contributions into one on-chain update with only $O(d)$ on-chain operations, independent of $m$. This significantly reduces the monetary cost of on-chain updates by $m$-fold via amortization.

==> alg/alg-prior-pot.tex <==
\begin{algorithm}
    \caption{Decentralized Powers-of-Tau Update}\label{alg:pot-update}
    \begin{algorithmic}[1]

    \Procedure{$\fun{ContractSetup}$}{}
    \Comment{Invoked by $\contract$}
        \State
        Sets $\pp = (\genone, \ldots, \genone; \quad \gentwo, \ldots, \gentwo ) \in \gpone^{n} \times \gptwo^{k}$
    \EndProcedure

    \Procedure{$\fun{Contribution}$}{}
    \Comment{Invoked by $\server$}
    \EndProcedure

    \Procedure{$\fun{ContractUpdate}$}{}
    \Comment{Executed on $\contract$}
        \State
        Sets $\pp = (\genone, \ldots, \genone; \quad \gentwo, \ldots, \gentwo ) \in \gpone^{n} \times \gptwo^{k}$
    \EndProcedure

\end{algorithmic}
\end{algorithm}
      
%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "../main"
%%% End:


==> draft.tex <==
\begin{align*}
  \mathsf{CheckInclude}(\mathsf{pk},
  \mathsf{st}_{\mathsf{Ser}},
  \mathsf{Inp}_{\mathsf{Ser}}
  )
\end{align*}


==> fig-overview-protocol-keynote.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.94\linewidth]{fig/aggregate-protocol.png}
  \caption{Overview of our Aggregation Protocol. It illustrates the workflow and shows the parties who involve in each algorithm.}
\label{fig:agg-protocol}
\end{figure}
\todo{Find a better way to present figure 4}


==> intro.tex <==
% !TEX root = main.tex

\section{Introduction}
\label{sec:intro}


% \todo{L: add applications that need PoT setup}

% \lucien{todo: change the paper template for uss}
% \lucien{todo: emphasize the ndss paper somewhere early on}
% \lucien{todo: mention the applications that needs pot}


Many cryptographic protocols depend on an initial setup to generate \emph{public parameters}. This is a critical step in preserving their security properties. 
This setup also creates an unwanted \emph{trapdoor} (also called a backdoor or toxic waste in the literature). If anyone learns this trapdoor, it would undermine the security properties of the system using those parameters. 
The \emph{powers-of-tau} is by far the most prominent example of such a setup. It is used in KZG polynomial commitments~\cite{aniket-polycommit-2010}, Verkle trees~\cite{verkle-tree}, fast proofs of multi-scalar multiplication (MSM)~\cite{msm-proofs}, the Danksharding proposal~\cite{danksharding} and  zk-SNARKs~\cite{sonic-2019, plonk-eprint-2019}. 
In fact, the increasing use of zk-SNARKS in the blockchain domain make powers-of-tau setup an indispensable tool within a variety of blockchain applications, including zk-rollups~\cite{rollups}, zkBridges~\cite{zkbridge} and privacy-preserving payment systems such as ZeroCash~\cite{zerocash}.  

In powers-of-tau, the public parameters ($\pp$) are defined as: 
{\small
\begin{align*}
  \pp
  % &= (\pp[1], \pp[2]) \\
  = (&\tau \genone, \tau^2 \genone, \ldots, \tau^n \genone; 
   \tau \gentwo, \tau^2 \gentwo, \ldots, \tau^k \gentwo )
% \\ &=  (a_1 B_1, a_2 B_1, \ldots, a_n B_1; b_1 B_2, \ldots, b_k B_2)
\in \mathbb{G}_1^n \times \mathbb{G}_2^k
\end{align*}
}
% \todo{Mohsen: I find the notation to be confusing, it looks like a citation at the moment, maybe subscripts is better if all agree.
% L: subscript is used to index the pp, and [i] is used to index the elements inside pp.}
Here, $\genone$ and $\gentwo$ are the generators of elliptic curve groups $\mathbb{G}_1$ and $\mathbb{G}_2$, respectively.  
We hereby denote the value $n+k$ as the \emph{number of powers-of-tau}, where 
the value $\tau$ is the trapdoor. 
\pedro{Supporting a large number of powers-of-tau is crucial for enhancing the expressiveness of an application using $\pp$. For example, in zk-SNARKs, the number of powers-of-tau dictates how complex the statement of the proof can be.}
To ensure the security of an application using $\pp$, it is crucial that $\tau$ is generated randomly and remains unknown to anyone. 
As a straightforward solution, one could rely on a trusted party to create $\pp$ in a so-called \emph{trusted setup}. 
This party selects $\tau$ at random, generates $\pp$, and deletes $\tau$ (and the randomness used to create it) as soon as the generation of $\pp$ is completed. 
However, trusted setups are not desirable in practice for decentralized applications as finding a universally accepted trusted party can be challenging.
% \todo{Panos: Why do we want to explicit mention the randomness that creates tau (which itself is random)? (such randomness is usually mouse pointer movements + system randomness etc. so it is considered "destroyed" anyway)
% L: we want to show we are well-educated cryptographers :)}

% \todo{there is a disconnection between the previous paragraph  and this paragraph} 
Given this problem, there is a clear motivation for a distributed protocol for \pedro{efficiently} generating power-of-tau parameters, which allows multiple users to participate.
Realizing such a protocol requires a key observation about the powers-of-tau $\pp$ is that it is \emph{re-randomizable}. 
Given $\pp$ and without knowing $\tau$, one can produce a new string $\pp'$ by choosing a new random value \pedro{$r$}  
and multiplying each component of $\pp$ by an appropriate power of 
\pedro{$r$}, more concretely: 
% \begin{align*}
%   \pp'  % &=  (\pp'[1], \pp'[2]) \\
%   = (&\tau' \cdot \tau \genone, \tau'^2 \cdot \tau^2 \genone, \ldots, \tau'^n \cdot \tau^n \genone;
%   \\&\tau' \cdot \tau \gentwo, \tau'^2 \cdot \tau^2 \gentwo, \ldots, \tau'^k \cdot \tau^k \gentwo )
% % \in \gpone^n \times \gptwo^k
% \end{align*}
{\small
\begin{align*}
  \pp'  % &=  (\pp'[1], \pp'[2]) \\
  = (&r \cdot \tau \genone, \ldots, r^n \cdot \tau^n \genone;
  r\cdot \tau \gentwo, \ldots, r^k \cdot \tau^k \gentwo )
% \in \gpone^n \times \gptwo^k
\end{align*}
}
% \\ &=  (a_1 \genone, a_2 \genone, \ldots, a_n \genone; b_1 \gentwo, \ldots, b_k \gentwo)
% Here, the new trapdoor becomes $\tau' \cdot \tau$ which is secure as long as \emph{either} $\tau$ or $\tau'$ are unknown and \emph{neither} is zero. 
Here, the new trapdoor becomes $r \cdot \tau$, which is secure as long as \emph{either} $\tau$ or $r$ are unknown and \emph{neither} is zero. 
% \todo{L: I'm think using $r$ is better than $\tau'$ because $\tau'$ should be representing the entire trapdoor value $r_1 ... r_m$ but not a multiplicative share of it.}
This re-randomizability property of powers-of-tau permits a relatively simple serial MPC protocol (also called \emph{ceremony}): the $i$-th user in turn randomizes the public parameters with their own chosen value \pedro{$r_i$}.  
As long as each participant correctly re-randomizes the $\pp$ from the previous user and at least one of the participants destroys their value \pedro{$r_i$} (and the randomness used to draw it), the cumulatively constructed public parameter will be secure. 

However, realizing such a ceremony in practice presents several challenges: 
\emph{(i)} all participants should agree on the final value of $\pp$ (\emph{consensus}); 
\emph{(ii)} each participant should only be able to re-randomize the current $\pp$ and not simply replace it with one for which the trapdoor is known to them (\emph{validity}); 
\emph{(iii)} the final $\pp$ should be available for all participants, as well as the history of prior versions for auditability (\emph{data availability}); 
\emph{(iv)} it should not be possible to prevent any participant from contributing to the ceremony (\emph{censorship resistance}). 
% \todo{Panos: If we are short on space we can merge this paragraph with the state of the art in I-A since it is not us who solve these anyway}
\todo{Pedro: Minor: If space and time left, we could:\\
- in (ii) why a user could simply "replace $\pp$ for one it with one for which the trapdoor is known to them"\\
- divide (iii) into two properties: $\pp$ should be available (data availability); the history should be verifiable (verifiability)}
\subsection{State-of-the-art and Goals}

Nikolaenko et al.~\cite{boneh-pot-2024} recently proposed a \emph{first truly decentralized and permissionless setup ceremony} for powers-of-tau. 
They observed that one can leverage a smart contract in a blockchain with expressive smart contracts (like Ethereum)  to coordinate the contributions of different participants of the ceremony. Upon receiving a contribution from a participant, the smart contract 
first checks its validity and 
then stores it as the last valid $\pp$. 
In doing so, this approach seamlessly leverages existing blockchain platforms to achieve part of the desired properties. 
In particular:  
\emph{(i)} consensus is inherently provided by the blockchain; 
\emph{(ii-iii)} the validity of each contribution as well as data availability are ensured by the smart contract itself; 
\emph{(iv)} the permissionless nature of existing blockchains makes them naturally resistant to censorship.  


However, the validity check required by the smart contract has a cost in terms of gas (i.e., the fee that the user needs to pay in Ethereum to execute the contract) that is linear in the number of powers-of-tau. 
{More significantly, these operations involve costly elliptic curve group operations, making it expensive for users to contribute}.
% \todo{L: But is it ``probhibitively expenisve?'' We are only reducing the gas cost by 10$\times$. If they are that expensive, we are not that far away D: remove probhibitively}
% This makes their approach very expensive in practice for users to contribute.
For instance, even for contributing a \pedro{$\pp$ with a} small number of powers-of-tau \pedro{e.g. $n+k = 1024$ elements}, a user's contribution will require $11,500,000$ gas (i.e., \$315 as reported in~\cite{boneh-pot-2024}).  
Note that limiting the number of powers-of-tau in $\pp$ restricts the applications for which the  generated $\pp$ can be used. 
For instance, in zk-SNARKS, the size of the statement that can be proven depends on the number of elements within powers-of-tau (i.e., fewer \pedro{values of $n+k$} can only work with small statements).

% \todo{pedro: Can we put a concrete example of why is really that bad that $n+k$ is 1024 in the case of Boneh?  D: added a sentence in blue} 

% \todo{We should highlight that boneh's construction cannot run efficiently on evm based}

In this state of affairs, the goal of this work is to answer the following question: 
\begin{center}
    \emph{Is it possible to devise a decentralized setup ceremony that permits a larger number of powers-of-tau while maintaining consensus, validity, data availability, and censorship resistance?}
\end{center}

\iffalse
Many cryptographic protocols, such as KZG polynomial commitment~\cite{aniket-polycommit-2010}, SNARK based on KZG polynomial commitment~\cite{sonic-2019, plonk-eprint-2019}, and the Danksharding proposal~\cite{danksharding}, require a trusted setup of a common reference string, known as
``Powers-of-Tau'' (PoT). This string is in the form of:
\begin{align*}
  \pp &=  (\pp[1], \pp[2])
  \\ &= \left( \tau B_1, \tau^2 B_1, \ldots, \tau^n B_1; \quad \tau B_2, \ldots, \tau^k B_2 \right)
% \\ &=  (a_1 B_1, a_2 B_1, \ldots, a_n B_1; b_1 B_2, \ldots, b_k B_2)
\in \mathbb{G}_1^n \times \mathbb{G}_2^k
\end{align*}
Here, $\gpone$ and $\gptwo$ are elliptic curve groups of prime order $p$ with generators $\genone$ and $\gentwo$. $n$ and $k$ are the predefined degrees required by the protocol instance. (In practice, $n \gg k$, so we can simplify $O(n + k)$ to $O(n)$).

The secrecy of $\tau \in \Zp$ is crucial, as anyone with knowledge of $\tau$ can compromise the security of the cryptographic scheme using this PoT string. Both $\tau$ and the randomness used to derive it are treated as toxic waste: they should be deleted as soon as the generation is completed, and the randomness should never be shared to prevent anyone from reconstructing $\tau$.

To reduce the chance of $\tau$ being leaked, most setups are conducted as a ceremony where numerous participants gather to contribute their randomness to $\tau$. To boost public confidence in the secrecy of $\tau$, most setup ceremonies adhere to the ``the more-the-merrier'' principle: the more participants contributing their randomness to $\tau$, the less likely $\tau$ will be leaked.
% To avoid anyone from learning $\tau$,

\pparagraph{MPC-based Setup Ceremony}
One strategy to reduce the risk of anyone discovering $\tau$ is to allow multiple parties to run a multiparty computation (MPC) protocol to compute the PoT string.
The MPC protocols are designed so that as long as one participant is honest,
$\tau$ will remain secret.
However, MPC-based protocols come with several drawbacks:
\begin{itemize}
    \item Efficiency: MPC protocols with a high tolerance for malicious parties typically entail significant computation and communication overhead. This overhead increases with the number of parties, limiting the number of participants.
    \item Synchronization Requirement: MPC protocols typically require parties to operate synchronously and struggle to handle aborts. If one party becomes unresponsive, the entire computation may need to be restarted.
    
    \item Censorship: 
    The parties can exclude anyone from the ceremony to prevent others from contributing randomness to $\tau$.
\end{itemize}

Efficiency and Synchronization requirements together limit the number of participants.
But the outstanding issue here is censorship.
% is perhaps the most outstanding issue.
By excluding other contributions, a group of malicious parties can fully control the randomness used in the ceremony and reconstruct $\tau$.

\pparagraph{Decentralized Setup Ceremony}
To address this, a decentralized setup ceremony is proposed to prevent censorship.
The idea is to conduct the ceremony on a smart contract on a permissionless blockchain, allowing anyone to contribute randomness to the PoT string.
Each contribution on the smart contract involves two steps:
1) the contributor updates the previous $\pp$ to a new $\pp'$ and upload it on-chain; and
2) the contributor provide a proof that $\pp'$ is a valid update from $\pp$, which the smart contract verifies immediately.
% The construction requires on two ideas:
% sequential update on PoT and proof of correct update (we will explain them soon.)

The second step is particularly expensive because the verification protocol~\cite{boneh-pot-2024} requires elliptic curve scalar multiplication (ECMult) $O(n + k)$ times, where $n + k$ is the total number of degrees in $\pp$.
For instance, Ethereum's transaction gas limit of $30$ million can only handle updates for PoT string with a total degree of $2048$.
In practice, applications usually need $\pp$ with degrees ranging from $2^{12}$ to $2^{20}$.
Such high on-chain computation costs limit the degrees of $\pp$ generated from the ceremony and discourage contributors due to the high monetary cost of updates.

Another issue is the high total on-chain computation cost.
Since every update needs to be presented and verified on-chain, the total cost is $O(n \cdot m)$ for $m$ contributions.
This results in the community cumulatively wasting a significant amount of resources for the ceremony.
\fi 

\subsection{Our Contributions}
\input{tb-rel-cost-cmp}
In this work, we answer this question in the affirmative. 
We propose a novel decentralized ceremony that significantly reduces the on-chain cost for users to contribute. 
This approach allows for 
\emph{(i)} a larger number of powers-of-tau; 
and 
\emph{(ii)} encourages more contributors, 
\todo{Pedro: What do you mean here?} which is crucial to increasing confidence in the secrecy of the trapdoor. 
In particular, our contributions are as follows:
% Our contributions are as follows:

\begin{compactitem}
  \item Working under the optimistic assumption,
  \todo{Pedro: What is the optimistic assumption? (I think I know, but the reader wouldn't know here, I think)}we propose an efficient fraud-proof protocol that enables us to
  % decouples storage and verication on the smart contract, reducing
  reduce the gas consumption of~\cite{boneh-pot-2024} by an order of magnitude, enabling setup ceremonies for larger $\pp$s.
  % constant size fraud-proof that is compatible with \cite{boneh-pot-2024}
  \todo{L: fraud proof is not constant size because we have Merkle proof that is $O(\log n)$}
  \item We present a proof aggregation protocol that enables a coordinator to batch $m$ updates into one $\pp$ and a constant-size proof. 
  \todo{Pedro: What is this proof? we have not explained it before?} Each batched update requires only $O(n)$ on-chain computation, in great contrast to the naive batching's $O(n \cdot m)$ on-chain computation.
  \todo{Pedro: $n$ is used before for $\mathbb{G}_1^n$. What is $n$ here?} \panos{I think $n$ is basically $n+k$}
  \todo{Pedro: Shall we say that our approach is asymptotically better than the previous work?}
  % or a  $O(n + m)$
  % off-chain proof aggregation
  \item We implemented our fraud-proof protocol and demonstrated that it is $16\times$ more efficient than other state-of-the-art on-chain solutions~\cite{boneh-pot-2024}.
  Our protocol supports a parameter size of $2^{15}$, which is sufficient for applications like ProtoDanksharding~\cite{eip4844}, whose targeted sizes of $\pp$ are $2^{12}$ to $2^{15}$.
  \item We prove the security of our proof aggregation scheme in the algebraic group model (AGM). Our aggregation scheme is built like a variant of BLS signature, which notoriously suffers from ``rogue key" attacks~\cite{proof-of-possion-bls}.
  We provide rigorous security definition that captures such attacks and prove the security of our scheme that has equipped with proper defense.
  \todo{Pedro: I am not sure I understand the last bullet}
  % provide model the  analyze the security of our scheme to show that it is immute from
% \todo{L: highlight that we can handle a PoT with degree $n = 2^{14}$ (or $2^{15}$), which is sufficient for applications eg., xxx D: removes when you think it is okay}
% \item security analysis using algebraic group model (AGM)
\end{compactitem}
% \todo{Pedro: I am here with my pass}
% \todo{Panos: we need to expand the 4 bullets above}
\Cref{tb:rel-work} shows a brief comparison with related works.

\todo{Pedro: general comments for this section:\\
 - Shall we clearly state that on-chain and off-chain protocols are two different proposals/contributions?\\
 - Add forward pointer to the section later in the paper where each "contribution" is spelled out}

\subsection{Our Contributions}
\pedro{
In this work, we positively answer this question. For this, our contributions are as follows:
}

\pedro{
First, we introduce SYSNAME, a fully decentralized and permissionless setup ceremony. Unlike the approach in~\cite{boneh-pot-2024}, where each $\pp$ update is proactively checked for two conditions before acceptance -- (i) the contributor knows the value $r$ used in the contribution, and (ii) the proposed $\pp$ is well-formed -- SYSNAME's key innovation is a fraud-proof protocol that shifts the paradigm for creating $\pp$. In SYSNAME, each proposed $\pp$ is only checked for condition (i) before acceptance, while condition (ii) is not proactively verified. If  a user \emph{a posterior} identifies an update as invalid under condition (ii), they can submit a succinct fraud proof. If the contract verifies this proof, it rejects the invalid $\pp$ update and reverts to the previous valid update.
}

\pedro{This paradigm shift allows us to design the fraud-proof protocol in a way that significantly reduces the gas consumption compared to~\cite{boneh-pot-2024}. This reduction enables setup ceremonies with a larger number of powers-of-tau while maintaining key properties such as consensus, validity, data availability, and censorship resistance.}

\pedro{ Second, to further enhance the efficiency of SYSNAME, we introduce an extension called SYSNAME-EXTENSION. In this system, users do not submit their $\pp$ and proof for fact (i) directly to the contract. Instead, they send them to an untrusted coordinator, who collects and forwards them to the contract. A key innovation here is our proof aggregation protocol, which allows the coordinator to batch $m$ tuples of the form ($\pp_j$, $\pi_j$)—where $\pp_j$ is the contributed $\pp$ and $\pi_j$ is the proof for fact (i)—into a single $\pp^*$ and a proof $\pi^*$ of size $O(\log(m))$.
When the coordinator submits $(\pp^*, \pi^*)$ to the contract, the contract verifies $\pi^*$ and accepts $\pp^*$ as the latest contribution. As with SYSNAME, $\pp^*$ is not proactively checked for validity under fact (ii), so users can still challenge its validity later using the fraud proof designed in SYSNAME.
SYSNAME-EXTENSION reduces the on-chain cost from $O((n+k) \cdot m)$ -- which would be required to store and process $m$ individual contributions -- to $O(n+k + \log(m))$. This makes the gas cost on-chain to only scale logarithmicly on the number of contributions the coordinator batches off-chain. We prove the security our proof aggregation protocol in the algebraic group model (AGM). 
}

\pedro{Third, we implemented SYSNAME and SYSNAME-EXTENSION and our performance evaluation shows that our approach is 16$\times$ more efficient that the current state-of-the-art solution~\cite{boneh-pot-2024}. More concretely, the efficiency boost of SYSNAME and SYSNAME-EXTENSION allows to create a $\pp$ with a number of powers-of-tau of $2^{15}$, thereby enabling for the first time its usage in applications like ProtoDanksharding~\cite{eip4844}, that requires $\pp$ with a number of powers-of-tau between $2^{12}$ and $2^{15}$. }

\subsection{Our Solution}
We aim to reduce the on-chain operation cost, making the ceremony economically accessible for more contributors, and thereby increasing confidence in the secrecy of $\tau$.

\subsubsection{Efficient Fraud Proof}
\todo{L: somehow we have a wrong impression that fraud proof is constant size but it's not. The pairing operation is constant but Merkle proof is not constant but $O(\log n)$}
To achieve this, we propose a fraud-proof protocol that reduces the number of on-chain elliptic curve multiplication and pairing equality check operations to a small constant number. Instead of \pedro{having a contract that explicitly verifies every update of $\pp$ as in~\cite{boneh-pot-2024}},  the contract optimistically assumes
each update is valid.
If anyone successfully challenges a previous $\pp$ using a fraud-proof,
the contract will revert the state to the $\pp$ immediately before the invalid $\pp$.
Importantly, our fraud-proof mechanism is not only efficient but is also decoupled from the update. 
\todo{Pedro: what does it mean "is also decoupled from the update"?}
As each update is now merely for storing the new $\pp$ and some correctness proof,
\todo{Pedro: What is the correctness proof?} the on-chain cost is significantly reduced.
This allows the contract to manage a ceremony \pedro{to create $\pp$ with a large number of powers-of-tau as required by}  practical applications and no longer heavily constrained by the gas cost.

\subsubsection{Aggregatable Contribution Proof}
\label{subsec:sol-agg-prf}
Despite the above improvement, on-chain asymptotic costs remain $O(n \cdot m)$ for $m$ contributors, as each contributor still needs to store their $O(n)$-size $\pp$ with $O(n)$ gas for the smart contract to read this input. 
\todo{Pedro: Now I kind of understand that the value $n$ is overloaded here meaning that we are using $n$ and $n + k$ to denote the same?}
% and proofs for the smart contract to verify.
% \todo{Why? Not clear what the costs after only the fraud proof are. L: added explanation}
Our goal here is to reduce the total gas costs
% to $O(n + m)$ or  
to $O(n)$, \ie, independent of $m$.
Therefore, we design an aggregatable contribution proof system on the validity of the update.
The main idea is to move the bulk of the computation off-chain and only upload the aggregated updated $\pp'$.
\todo{Pedro: I am confused here: what is the "computation" that is referred here? Before in 1.3.1 says that validity is not checked, instead a fraud proof is used if something is wrong}
Instead of having each contributor upload their own update on-chain, 
we propose a (trustless) coordinator that aggregates the contributors' updates and proofs, only needing to upload the final $\pp$ and an aggregated proof requiring a few group elements, resulting in a total on-chain cost of $O(n)$.
This protocol can significantly reduce the participation cost via amortization. 
\todo{Pedro: expand on amortization here, what do you mean?}
Furthermore, our protocol remains censorship-resistant; in the event of an operator \panos{Who is the operator?} denying a contributor's update, the contributor can go to another operator or update $\pp$ on-chain independently. 
\todo{Pedro: I would move this last point about censorship resistance to a discussion at the end. The rest is already complex enough to parse}

However, our aggregatable proof protocol also needs to incorporate the following required properties:
% However, there are three significant challenges in such an aggregatable proof system that need to be addressed:
%\todo{Panos: Which are the 3 challenges? I see more than 3 below. L: modified}

\pparagraph{Oblivious Accumulated Randomness}
In the validity proof of an update, a contributor needs to prove their knowledge of the random value $r$ that is multiplied to the prior $\pp = (\tau \cdot \genone, \ldots)$ to get the updated $\pp' = (r \cdot \tau \cdot \genone, \ldots)$. This ensures they cannot ``reset'' the $\tau$.
The contributor, as the prover, knows the randomness and can use Schnorr's $\Sigma$-protocol~\cite{crypto-1989-1727} and BLS-style proof of possession~\cite{proof-of-possion-bls} to prove its knowledge of $r$.
However,
when a coordinator is aggregating the updates, the new $\pp'$ becomes $(r_{1} \ldots r_{m} \cdot \tau \genone, \ldots)$.
None of the parties, including the coordinator or any contributor\pedro{on their own}, knows the accumulated random value $r_{1} \cdot \ldots \cdot r_{m}$, and for the secrecy of the $r$'s,
we must not allow any individual to learn that.
It means that
Schnorr's $\Sigma$-protocol and BLS-style proof of possession protocol are not useful in our case. 
\todo{Pedro: I would add here the argument on why the collaborative NIZKs is not a desirable approach either}
Therefore, we design an aggregatable proof that allows each contributor to ``add'' their witness to a constant-size proof without sharing the witness with anyone else.
% as if part of their update.

\pparagraph{Fire-and-Forget Aggregation}
In a ceremony, the contributors may wish to complete their contributions \pedro{ideally in a single shot message, avoiding an interactive protocol with the coordinator or other contributors.} %quickly and not maintain a long-term connection with the coordinator or other contributors.
Moreover, we want to allow the contributors to join and leave at any time.
% Still, we want the coordinator be able to aggregate their proofs into a constant-size proof.
General multi-party computation (MPC) or zero-knowledge proof techniques are ruled out as they require parties to stay online and run the protocol in a synchronized manner.
% A na\"ive solution is to use multi-party computation (MPC) to compute the aggregated proof of knowledge on $r$s.
%General MPC techniques [cite] require the parties stay online and run the protocol in synchronized manners.
% If some parties
% It will require all the contributors to stay online and run the prtocol
Some parties' abortion can lead to the re-execution of the entire protocol.
General zero-knowledge proof systems require a single prover to know the entire witness, \ie, $r_{1}\ldots r_{m}$, which is not feasible for us.
Recursive zk-SNARK (with transparent setup), which provides a zk-SNARK proof about multiple zk-SNARK proofs, might achieve the desired functionality, but the proof might be expensive to compute and prohibitively expensive to be verified on a smart contract due to the logarithmic-size of proof.

In contrast,
the contributor in our proof system
sends the proof (and $\pp'$) to the coordinator,
who then passes them to another contributor along with the $\pp'$. 
Importantly, 
the server does not need to communicate with previous contributors again to complete the proof, achieving our ``fire-and-forget'' property.

\todo{Pedro: Shall we merge the two previous paragraphs?}

% \todo{Panos: can we just call this "non-interactive aggregation"? or "asynchronous aggregation"? "non-interactive" is not entire accurate because the next contributor needs the proof from the prior contributor to aggregate. "asynchronous" is ambiguous and usually implies situation that invokes abortions
% Panos: sure but there's still no back and forth communication (i.e. "interaction") - just trying to find a more standard term than "fire and forget"
% }

\pparagraph{Succinct Proof for On-Chain Verification}
The succinctness of our aggregated proof and the efficiency of verification are paramount for practicality.
Our conservative estimation on the on-chain cost of the prior Schnorr's $\Sigma$-based-protocol~\cite{boneh-pot-2024} is ${>}10,000$ gas per contributor.
In Ethereum's KZG Ceremony for PoT, it has $m {>} 140,000$ contributors, 
which translates to ${>}1.4$ billion gas consumption, which is ${>}46\times$ higher than the gas limit per block in Ethereum's blockchain.
% and ${>}13,000$ USD\footnote{As of 10 July, 2024}.
% https://www.cryptoneur.xyz/en/gas-fees-calculator?usedGas=1400000000&txnType=Custom&gasPrice=standard

In our scheme's on-chain verification,
the verification in our scheme is inexpensive as
the smart contract only needs to
a proof consisting of a $3$ group elements and can be verified with only $3$ pairing operations.
% \todo{add concrete gas cost.}

\pparagraph{Proof of Randomness Inclusion}
Since multiple contributions are combined into one, the final $\pp$ and the proofs are different from what the contributors provided to the coordinator. A malicious coordinator could discard a contributor's randomness, yet deceive them into believing it's included. We need a way for each contributor to confirm their contribution are indeed included in the final $\pp$ presented on the blockchain.
% \todo{Panos: Isn't the above about just preserving censorship resistance?
% L: here is the subtlety: our (or my) intepretation of censorship is whether someone can stop someone from joining the ceremony, and when one is being denied, it knows. However, without randomness inclusion proof, someone might be denied unknowingly and thought he is participating. }

Letting contributors be able to verify the inclusion of randomness is important for censorship resistance. Should a contributor fail to provide an inclusion proof,
a contributor can join the batched contribution with another coordinator, instead of having a ``false sense of contribution.'' \panos{This sentence does not read well. What are we trying to say here?}
\lucien{It should be false "sense" of contribution, but the word sense was missed.}

\pparagraph{Efficient Randomness Inclusion Verification}
To verify randomness inclusion,
a contributor obtains a proof of randomness inclusion from the coordinator off-chain and verifies it locally.
If the coordinator refuses to provide the inclusion proof, a contributor can initiate another contribution with a different coordinator or submit its contribution on-chain independently.
\todo{Pedro: With the larger number of powers-of-tau, can a contributor do this really? isn't too expensive now?}

Importantly,
a contributor does \emph{not} need to verify the proofs on other coordinators.
This is a significant contrast to prior PoT techniques where a contributor needs to read the entire transcript of the ceremony to verify its validity. 

% \todo{Panos: Maybe we can merge the above 2 paragraphs into a single one like "Designing an efficient proof for censorship resistance"}

% to avoid confusion


% \pparagraph{Aggregatable Zero-knowledge Proof}
% To resolve all these issues at once, we provide an aggregatable zero-knowledge proof system tailored for batched contributions.
% Our system allows each contributor to ``add'' their witness on a constant-size proof without sharing the witness to anyone else. The contributor then sends the proof to the coordinator, who then passes it to another contributor and needs not to communicate with previous contributors again to complete the proof, achieving our ``fire-and-forget'' property.

% The verification of randomness inclusion is decoupled from on-chain verification.
% A contributor can obtain a proof of randomness inclusion from the coordinator off-chain and verifies it locally.
% Should the coordinator refuses to provide the inclusion proof, a contribution can start another contribution with another coordinator or submit its contribution on-chain by itself.

 % \todo{Rearrange the above}

% \todo{L: a contributor can go to other server}
% \todo{No need for consensus within a server/coordination. L: I forgot what I meant}
% \todo{Highlight our security proof as a contribution}

% requires each contributor any single party to know the entire secret randomness
% \todo{highlight the challenge that the server cannot know all the witness to construct the proof.}
% \todo{highlight our fire and forget property.}









%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End:


==> overview.tex <==

\section{Technical Overview}

In this section, we present an overview of our proposed components and explain how they can be integrated to make the PoT ceremony practical.



\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{fig/protocol-overview.pdf}
  \todo{Pedro: Maybe cross out the wellform check instead of red highlight for clarity?\\
  - We could also add "Fraud-Proof Mechanism" and "Aggregatable Contribution"\\
  - One question here is: are these two things interchangeable? In other words, what happens when after $\pp_{t-1}$, we enter the aggregation coordinator and then another user submits a different $\pp_t$ on-chain? I imagine that they are exclusive epochs/phases? Maybe clarify (e.g., by adding another submission of $\pp$ on-chain to the right?}
  \caption{Number 1, highlights the overview of our Fraud-Proof mechanism. In the first step, the contract only performs the possession and the degeneration check. However, compared to~\cite{boneh-pot-2024}, the contract does not perform the expensive well-formedness check. If $\pp_t$ is ill-formed,  $\contract$ can verify a fraud-proof $\pi_{\mathtt{fraud}}$ with $O(\log(n+k))$ gas consumption in the consecutive blocks and reverting back to $\pp_{t-1}$. Number 2, provides an overview of our Aggregatable Contribution Scheme. In this approach, a coordinator receives contributions from multiple parties, verifies the contributions off-chain, aggregates the proof, and submits the latest $\pp$ along with proof for performing the possession and degeneration checks on-chain. }
\label{fig:protocol-overview}
\end{figure*}
\todo{L:
  1) we can remove the cost in \Cref{fig:protocol-overview} because \Cref{tb:fraud-cost} subsumes the cost comparision.
  2) we might add another operator (now we can changing the name) to highlight we support multiple operators.
  3) we should mention a user can join another oeprator or be an operator in face of censorship.
  4) Also, this fig and caption is taking too much space}

\subsection{Fraud-Proof Mechanism}
\label{subsec:fraud-proof-overview}
\label{subsec:fraud-overview}


\input{tb-fraud-cost}


We begin by focusing on the scenario where a single contributor attempts to update the PoT string from
$\pp_{t-1}$ to $\pp_{t}$.
\Cref{tb:fraud-cost} shows our concrete gas cost compared to \cite{boneh-pot-2024}'s.
Our goal is to efficiently perform a $\checktwo$ on $\pp_{t}$ through a fraud-proof mechanism.
Part~\circled{1} of~\Cref{fig:protocol-overview} illustrates this mechanism.
\lucien{Part~\circled{1} is only showing the cost and the rewind mechanism, but not illustrating how it works}


% We illustrate our fraud-proof mechanism in~\Cref{fig:fraud-overview}.

\pparagraph{Optimistic Assumption}
To avoid prohibitively expensive verification in ceremonies with a practical number of \pedro{number of powers-of-tau} (e.g., $n + k > 2^{12}$), we drastically reduce the verification cost through an optimistic assumption. The contract accepts an update $\pp$ by only performing $\checkone$ and $\checkthree$ without verifying the $\checktwo$.

However, if anyone discovers an invalid historical $\pp_t$, they can submit a challenge to the contract. If the challenge is deemed successful, the contract rewinds its state to the $\pp$ immediately preceding the invalid one, i.e., $\pp_{t-1}$, and voids all subsequent updates. This approach incentivizes contributors to verify prior updates and challenge invalid ones, thereby preventing their efforts from being wasted.

Nevertheless, in the worst-case scenario where an invalid $\pp$ is discovered and a challenge is raised, the contract still needs to perform the expensive $\checktwo$ for verification. This is necessary because while the $\checkone$ and $\checkthree$ are efficient, they do not fully guarantee that $\pp$ is well-formed. 
The $\checktwo$ serves as a final safeguard to ensure the integrity of the updates when an issue is detected.

To address the potentially high cost of this verification, we propose a new fraud-proof mechanism that reduces the verification cost to merely reading four group elements and performing two pairing equality checks, regardless of $n$ and $k$, plus $O(\log (n+k))$ hashing operations, whose gas cost is substantially lower than that of a pairing equality check.


% \begin{figure}[b]
%   \centering
%   \includegraphics[width=0.9\linewidth]{fig/fraud-overview.pdf}
%   \caption{An overview of our Fraud-Proof Mechanism. In this toy example, if $\pp_1$ is ill-formed, $\contract$ can verify a fraud-proof $\pi_{\mathtt{fraud}}$
%     % to verify if $\pp_1$ is ill-formed
%     with $O(\log n)$ gas consumption.}
% \label{fig:boneh-overview}
% \end{figure}

% The two pairing equaitly checks are
\pparagraph{Pairing Equality Checks}
The first pairing equality check is:
\begin{align*}
    e(P_1, \gentwo) \isequal e(\genone, Q_1)
    % e(P_{\idxill}, \gentwo) &\isequal e(\genone, Q_1)
\end{align*}
where $P_1$ and $Q_1$ are extracted from $\pp = (P_1, \ldots, P_n; Q_1, \ldots, Q_k)$.
If this equality does not hold, the contract accepts the fraud-proof and deems the challenge successful.

If this equality holds, we can safely assume that $P_1 = \tau\genone$ and $Q_1 = \tau \gentwo$ for some $\tau \in \Zp$.
Given this assumption, if $\pp$ is ill-formed but still passes the above equality test, it must be structured as:
\begin{align*}
    \pp = (\tau\genone, \ldots, \tau^{i-1}\genone, r\genone, \ldots; \quad \tau \gentwo, \ldots )
\end{align*}
where the $i$-th item in the array for $\gpone$ is incorrect, i.e., $r \neq \tau^i$ for an index $i > 1$, and it is the first incorrect item in $\gpone$. This implies that $P_{i-1} = \tau^{i-1}\genone$. Without loss of generality, we assume the error occurs in $\gpone$, though our approach also applies to errors in the array for $\gptwo$.

To prove the $i$-th item in $\gpone$ is incorrect, the prover submits the index $i$ to the contract, which then verifies the fraud-proof by computing
\begin{align}\label{eqt:ill-pairing-check}
    e(P_{i-1}, Q_1) \isequal e(P_i, \gentwo)
\end{align}

Given our assumption that $P_i \neq \tau^{i}\genone$, the above equality must not hold, because the left-hand side (LHS) is:
\begin{align*}
e(P_{i-1}, Q_1) =
e(\tau^{i-1}\genone, \tau \gentwo)
=\tau^{i} \cdot e(\genone, \gentwo)
\end{align*}
while the right-hand side (RHS) is:
\begin{align*}
    e(P_i, \gentwo)
    = e(r\genone, \gentwo) = r \cdot e(\genone, \gentwo)
\end{align*}
Thus, LHS $\neq$ RHS because $r \neq \tau^{i}$.

While there may be other incorrect items in $\pp$, it is sufficient to prove $\pp$ is ill-formed by demonstrating that just one item is incorrect.


\pparagraph{Storing $\pp$ as Vector Commitments}
% \pparagraph{Efficiency of Fraud Proof Verification}
% In the worst case, the contract $\contract$ needs to perform two pairing equality checks to verify a fraud-proof.
To execute the aforementioned checks, $\contract$ must access four specific group elements from $\pp$.
However, storing the entire $\pp$ values on-chain is expensive due to the high gas costs for storage slots for each update.% (i.e., 20,000 gas for each slot).
% \todo{M: I wouldn't put the paragraph title below. the previous point on efficiency is not completed. The point is half baked at this point}
% L: I changed the text inside for the heading. I think using VC is something worth highlighted as a heading
To address this,
% we use vector commitment $\compp$ to represent $\pp$.
% Instead of storing all elements of $\pp$,
$\contract$ only stores $\compp$, the Merkle root of $\pp$.
When a challenge is raised against the $\pp$, the challenger also provide a membership proof corresponding to $\compp$ for the relevant elements.
% within the  Merkle tree.
Computing $\compp$ require $O(n+k)$ calldata and hashing, which is an order of magnitude cheaper than storing the $\pp$.
To handle a challenge, $\contract$ can verify the membership proof with an insignificant gas cost of $O(\log(n+k))$ calldata and hashing.
\todo{Pedro: Add here a concrete number for comparison?}
% , which is orders of magnitude cheaper than storing the $\pp$.
% making it significantly more efficient than performing elliptic curve multiplication and pairing operations.
% \todo{add number comparisons}

Although $\contract$ no longer stores $\pp$ in its state, $\server$ and $\user$ can still fetch the historic $\pp$ from blockchain transaction history for fraud proof and setting up off-chain udpate.

% \todo{@lucien: check below, some pp changed to compp.}
\pparagraph{Non-Blocking Challenge Phase}
A naïve approach to the challenge mechanism might involve a dedicated fixed period for each $\pp$ update, during which no further updates occur.
However, this waiting period is unnecessary.
Instead, the next update can proceed immediately after the current one.
The contract inexpensively maintains a history of all $\pp$ states in the form of commitments $\compp$, allowing anyone to challenge any $\pp$ in this history.
The challenger specifies and index $\histidx$ to specify which $\compp$ to challenge.
If the challenge is successful, the contract reverts to the valid state  $\compp_{\histidx-1}$, and any subsequent updates must be proven as valid extensions from this corrected state. %the next $\pp$ should be proven to be a valid update built on top of $\compp_{\histidx-1}$.


% \todo{M: remove the next three paragraphs}
% \pparagraph{Efficiency of Fraud Proof Verification}
% In the worst case, the contract $\contract$ needs to perform two pairing equality checks. Additionally, it needs to read four elements from $\pp$ via membership proofs on $\compp$, which requires $O(\log n)$ calldata and hashing.
% \lucien{Mention how to optimize for locating the fraud position}

% \pparagraph{Non-Blocking Challenge Phase}
% A naïve approach to the challenge mechanism is to have a dedicated fixed period for each $\pp$ update.
% The subsequent update would have to wait until the end of the challenge period.
% However, this wait is unnecessary.
% After an update, the next update can occur immediately.
% The contract can store all the historic $\pp$ and allow anyone to challenge any $\pp$ in the history.
% The challenger can simply add an extra index $\histidx$ to specify which $\pp$ to challenge.
% If the challenge is successful, the latest $\pp$ will become $\pp_{\histidx-1}$,
% and the next $\pp$ should be proven to be a valid update built on top of $\pp_{\histidx-1}$.

% \pparagraph{Storing $\pp$ as Vector Commitments}
% Another concern is on-chain storage. Storing all past $\pp$s is expensive because, for every update, the contract needs to initialize
% $n + k$ empty storage slots, each of which costs $20,000$ gas.
% Our solution is to use a vector commitment $\compp$ to represent the $\pp$, and the contract only stores a $\compp$ for each update.
% % store $\pp$s in an array of vector commitments.
% For each update, the contract computes the commitment $\compp$ using a Merkle tree and only stores the root of it. When a challenge is launched against a $\pp$, it needs to submit the membership proof of $P_1, Q_1$ inside the corresponding $\compp$ Merkle tree.
% %If the first equality check passes, $P_{i-1}, P_{i}$.
% The on-chain computation cost to verify a membership proof is $O(\log (n+k))$, which is substantially cheaper than ECMult and pairing operations.

\todo{L: We move the paragraphs below to Discussion and leave a few high-level sentences here}
\pparagraph{Pinpointing the Ill-Formed Element}
% In \Cref{alg:local-ext-wellform},
\Cref{alg:local-ext-wellform} outlines a straightforward method to pinpoint the ill-formed element using $n + k - 2$ pairing operations.
The idea is to perform a pairing check on each pair $(P_{i-1}, P_{i})$ using \Cref{eqt:ill-pairing-check} and similarly for each pair $(Q_{i-1}, Q_{i})$.
% This cost is not significantly higher than that of the prior off-chain well-formness check (without identification),
% \ie, \cite{boneh-pot-2024}'s well-formness check, which requiers $n+c$ EC scalar multiplications and one pairing check,
% because EC scalar multiplication is about $7\times$ faster than pairing checks in local computation~\cite{eccbench}.

However, it is possible to reduce the computation cost by combining the well-formedness check from~\cite{boneh-pot-2024} with binary search, reducing the requirements to $n+k$ elliptic curve (EC) scalar multiplication and $\log_{2} (n+k)$ pairing checks.
%$n+k$ EC scalar multiplication and $\log_{2} (n+k)$ pairing checks by combining \cite{boneh-pot-2024}'s well-formedness check with binary search.
With this optimization, our pinpointing protocol's \mohsen{what is identification protocol? first time mentioned in this section} cost is only slightly higher than \cite{boneh-pot-2024}'s, which requires the same number of EC multiplication but only a single pairing operation.
%these protocols need the same number of ECMults, while \cite{boneh-pot-2024}'s requires only $1$ pairing operation. 
% (But their saving in off-chain pairing operation might need to be paid back during the on-chain verification for ECMulT over $\gptwo$.)
Nevertheless, since off-chain cost optimization is not our main focus, we present the simpler protocol here. 
\todo{Pedro: This is about some off-chain computation that challenger needs to do, right? I would write this in the discussion later to make this section clearer, and only add a forward reference here}
% This idea might accelerate the identification by ${\approx} 3\times$ because EC scalar multiplication is about $7\times$ faster than pairing checks in local computation~\cite{eccbench}.
% Nevertheless, we would rather focus on the on-chain cost and thus leave further optimization of off-chain for futher work.
% We do not formalize this idea because in off-chain computation, pairing checks is less than an order of magnitude slower than EC scalar multiplication~\cite{eccbench}.
% .
% We thus

\subsection{Aggregateable Contribution}
\label{sub:agg-contribution}
A key contribution of our solution is the use of a coordinator that collects contributions from multiple users off-chain and then submits only the final aggregated result on-chain. This process significantly reduces fees by minimizing the amount of data that needs to be recorded and verified on-chain. 


%We now shift our focus to how $\server$ can aggregate multiple validity proofs into one. Suppose the operator wants to aggregate the following $m$ updates:
The coordinator handles a sequence of updates:
\begin{align*}
    \pp_0 \to \pp_1 \to \dots \to \pp_m
\end{align*}
and submits the final state $\pp_m $ along with a \emph{constant-size} validity proof $\pi$, independent of  the number of updates $m$ or the parameters $n$ and $k$. 

\lucien{I would suggest phrasing the below as an observation because we brag about the reduction in the abstract (which hints the batched computation of $\checktwo$ as an contribution)}
This aggregation primarily impacts the \checkone, which is the only check aggregated by the operator. The \checktwo\xspace and \checkthree remain unchanged, as these checks focus on the final form of the aggregated result. remain the same since only the final form of the aggregated result is verified. The emphasis here is on ensuring that each contributor correctly possesses the randomness used throughout the aggregation process.

In part~\circled{2} of~\cref{fig:protocol-overview}, we illustrate how our solution leverages the role of multiple operators who collect contributions from different users off-chain. Each operator processes the contributions sequentially, updating the parameter $\pp$ off-chain and ultimately submitting the aggregated result on-chain. This method ensures that only the final state and compact validity proof $\pi$ are committed on-chain.

\todo{Pedro: I think we need to put clear that the ``only'' proof that is aggregated is the possession and non-degenerate check. The validity of pp is still not checked. \\
I think I would refer to the figure and put a concrete example of what we are doing here with e.g., 2-3 users and their contributions. \\
More concretely, I think Figure 1 is really nice to show what are the key ideas of the constructions, so we could use it to explain the idea to the reader at this level, before entering in the concrete proof (section 3.2.1)}
%By applying the fraud-proof protocols from~\cref{subsec:fraud-overview}, the contract can efficiently verify the final $\pp_m$ without being affected by the aggregation process.

% \begin{figure}
%   \centering
%   \includegraphics[width=0.94\linewidth]{fig/agg-overview.pdf}
%   \caption{An overview of our Aggregatable Contribution Scheme
%   }
% \label{fig:agg-overview}
% \end{figure}
% \todo{fix figure}
% Ideally, the operator should only submit the final $\pp_m$ and a constant-size validity proof $\pi$, whose size is independent of $m, n, k$.


% We begin with an observation that among the three validity checks, $\checktwo$ and $\checkthree$ can be trivially ``aggregated'' by letting the smart contract check only the final $\pp_m$.
% In fact, the purpose of a ceremony is to generate a structured string
% regardless the intermediate values,
% as long as the final form is correct and $\tau$ remains secret.
% Similarly, for $\checkthree$,
% we only need to check if the final $\pp$ is degenerated.
% Hence, we can trivially apply the fraud-proof protocol in Section~\ref{subsec:fraud-overview} for Check \# 2. For Check \#3, the contract can implement a fraud-proof protocol to spot if any of $\{P_i\}_i$ or $\{ Q_i \}_i$ is zero.

% Nevertheless, $\server$ and $\user$s still need to verify the intermediate $\pp$ off-chain to ensure they are updating
% a valid PoT; otherwise, the final $\pp$ might be ill-formed or degenerated.


\subsubsection{Strawman Aggregation Protocol}
\todo{i will change vk to aggregated public key ($\mathsf{AggPK}$).}
\todo{L: I would suggest changin the macro ($\vk, \prevk, \curvk$) because it will much easier if you want to change it to other notations later}

\pparagraph{Aggregating the Knowledge of Randomness}
As discussed, towards aggregating the proof for $\checkone$, we face the challenges mentioned in \Cref{subsec:sol-agg-prf}.
To address these challenges, we propose a BLS-style aggregatable proof scheme, which aggregates the proof using pairing's bilinearity.

For ease of exposition, we introduce our scheme gradually through different cases with increasing complexity.

\pparagraph{Single Contributor Case}
Suppose there is only one contributor $\user_{1}$. It samples a secret key $\sk$ and public key $\pk$:
\begin{align*}
\sk \sample \Zp \quad\quad \pk = \sk \cdot \genone \in \gpone
\end{align*}
Then it computes a $\pp$ exactly like the normal case: it samples $r \sample \Zp$ and update $\pp$ to $\pp'$ using $r_{1}$ as the random value.
To produce a proof of possession of $r$, it computes
\begin{align*}
\sigma = \sk \cdot \pp.Q_{1} = \sk \cdot r \cdot \gentwo \in \gptwo
\end{align*}
and outputs $\pi = (\pk, \sigma)$ as the proof.

For a verifier, \eg, $\contract$ or $\server$, to conduct $\checkone$,
the contributor submits $\pp$, the verification key $\vk = \pk$, and $\sigma$ to the verifier, who then verifies that
\begin{align*}
e(\vk, \pp.Q_{1}) \isequal e(\genone, \sigma)
\end{align*}
Correctness holds because
\begin{align*}
 e(\vk, \pp.Q_{1}) = e(\sk \genone, r \gentwo) =  e(\genone, (\sk \cdot r) \gentwo) = e(\genone, \sigma)
\end{align*}

Meanwhile, the secrecy of $r$ and possession of $r$ (by $\user_{1}$) are both gauranteed
by the $(n, k)$-Strong Diffie-Hellman Assumption.

% Now, $r$ is hidden in the scalar of a group element $\sigma_{1}$, so no other parties can learn $r$.
% Meanwhile, by the $(n, k)$-Strong Diffie-Hellman Assumption,
% a PPT adversary only has negligible probability to pass the above equality check.

\pparagraph{Two Contributor Case}
While the above construction already provides a new protocol for checking $\checkone$,
the most interesting aspect is how we can extend it to an aggregate protocol for multiple contributions.

% Suppose there is a coordinator $\server$ who collects the sequential contributions
% and have already received $\sigma$ and $\pk_{1}$ from $\user_{1}$.
% Furthermore, we assume there is a second contributor $\user_{2}$ who wants to contribute.

Now, suppose there is a second contributor $\user_{2}$ with random value $r$ and a key pair $(\sk', \pk') \in \gpone \times \gptwo$.
Firstly, $\user_{2}$ obtains the piror $\pp$ from $\user_{1}$ and computes $\pp'$ from $\pp$ with $r'$.

This time, the computation for $\checkone$'s proof is different.
$\user_{2}$ also obtains $\sigma$ from $\user_{1}$.
% $\user_{2}$ samples a secret-public key pair $(\sk_{2}, \pk_{2} = \sk_{2} \cdot \gentwo) \in \Zp^{*} \times \gptwo$,
% fetches $\sigma$ from $\server$,
and computes
\begin{align}\label{eqt:single-update}
  \sigma' = r' \cdot \sigma + \sk' \cdot \pp'.Q_{1}
\end{align}
and finally output $\pp'$ with $\pi' = (\pk', \sigma')$ as the proof.

Anyone with $\pk$ can verify this proof by computing
a new verification key $\vk \leftarrow \pk + \pk$ and checking
\begin{align}\label{eqt:single-pairing-check}
e(\vk, \pp'.Q_{1}) \isequal e(\genone, \sigma')
\end{align}
Correctness holds because
\begin{align*}
  e(\vk, \pp'.Q_{2}) &= e(\pk + \pk', r' r \gentwo)
  \\ &= e(\genone, (\sk + \sk') r' r \gentwo)
  % \\ &= (\sk_1 + \sk_{2}) r_{2} r_{1} \cdot e(\genone, \gentwo)
  = e(\genone, \sigma')
\end{align*}
% The last equality is due to
% $\sigma' = r_{2} \cdot (\sk_{1} \cdot r_{1} \cdot \gentwo) + \sk_{2} \cdot \pp'.Q_{2} = (\sk_{1} + \sk_{2}) r_{2} r_{1} \gentwo$.

Again, by the $(n,k)$-Strong Diffie-Hellman assumption, the above protocol gaurantees
i) the secrecy of $r_{1}$ and $r_{2}$ , and ii) $\user$ and $\user'$ joint possession of $r' \cdot r$.
% This proof also demonstrates $\user_{2}$'s knowledge of $r_{2}$ to $\server$. Again, by $(n,k)$-Strong Diffie-Hellman assumption,
% the probability for a PPT adversary coming up with $\sigma'$ without $r$ is negligible.
% There are two saliences of this protocols.

Meanwhile,
This protocol already achieve most we have promised:
i) the proof is aggregated into a constant-size proof ($\sigma'$ and $\vk$), which has only two group elements;
ii) it has the fire-and-forget property, as $\user_{2}$ needs not to interact with $\user_{1}$;
and iii) It produces a proof for the oblivious accumulated randomness because neither $\user_{1}$ and $\user_{2}$ knows $r' \cdot r$

% First, the proof for $\checkone$ still remains a constant size of two group elements ($\sigma'$ and $\vk$).
% Second,
% $\user_{2}$ can compute its proof without interaction with $\user_{1}$.
% It aligns with PoT's sequential update paradigm, where a contributor can leave upon finishing its contribution.

\pparagraph{Three or More Contributors Case}
Generalizing the above strawman scheme for more contributors is straight-forward.
% We list the procedures in \Cref{alg:strawman-single-update}.
A new contributor $\user'$ gathers $\pp$ and $\sigma$ from the previous contributor, updates $\pp$ to $\pp'$, and compute
new proof $\pi' = (\pk', \sigma')$ using \Cref{eqt:single-update}.
Anyone with the all the $\pk$s can verify this update using \Cref{eqt:single-pairing-check} with $\vk$ being the sum of all $\pk$s.

% \begin{algorithm}
%     \caption{Strawman Single-$\server$ Aggregate}\label{alg:strawman-single-update}
%     \begin{algorithmic}[1]
%     \Procedure{$\fun{StrawServerSetup}$}{}
%     \Comment{Invoked by $\server$}
%       \State Sets $\pp = (\genone, \ldots; \quad \gentwo, \ldots) \in \gpone^{n} \times \gptwo^{k}$
%       \State Set $\vk = \genone$, $\sigma = \genone$
%     \EndProcedure
%     \Procedure{$\fun{StrawOffContribute}$}{}
%     \Comment{Invoked by $\user$}

%     \State
%     Fetches $\pp, \sigma$ from $\server$

%     \State
%     Samples $r \sample \Zp^{*}$
%     \State
%     Computes $\pp \leftarrow \fun{UpdatePP}(\pp; r)$

%     \State
%     Samples $\sk \sample \Zp^{*}$ and computes $\pk = \sk \genone$

%     \State
%     Computes $\sigma \leftarrow r \cdot \sigma + \sk \cdot \pp.Q_{1}$

%     \State Outputs $\fun{StrawOffUpdate}(\pp, \sigma, \pk)$

%     \EndProcedure

%     \Procedure{$\fun{StrawOffUpdate}$}{$\pp', \sigma', \pk$}
%     \Comment{Exec on $\server$}
%     \State Computes $\vk^{*} = \vk + \pk$
%     \If{$e(\vk^{*}, \pp') = e(\genone, \sigma')$}
%       \State Sets $\pp \leftarrow \pp'$, $\sigma \leftarrow \sigma'$,  $\vk \leftarrow \vk^{*}$
%       % $\stkey \leftarrow \stkey || \pk$,
%       \State Outputs $1$
%     \Else
%        \xspace Outputs $0$
%     \EndIf
%     \EndProcedure

% \end{algorithmic}
% \end{algorithm}

% Suppose $\server$ stores $\pp_{i}$, $(\pk_{1}, \ldots, \pk_{i})$, and
% $\sigma = (\sk_{1} + \ldots + \sk_{i}) r_{1} \cdot \ldots \cdot r_{i} \gentwo$.

% % \lucien{Put the following into a algorithm figure (while emphasizing it is a strawman scheme)? or skip this generalization?}
% When the $(i+1)$-th contributor $\user_{i+1}$ wants to contribute, it fetches $\pp_{i}$ and $\sigma$ from $\server$.
% Then, $\user_{i+1}$ computes $\pp_{i+1}$ from $\pp_{i}$ with a fresh random value $r_{i+1} \sample \Zp$,
% generates a new key pair $(\sk_{i+1}, \pk_{i+1})$, and compute $\sigma' = r_{i+1} \sigma + \sk_{i+1} \cdot \pp_{i+1}.Q_1$.
% Finally, $\user_{i+1}$ sends $\pp_{i+1}$ and $(\pk_{i+1}, \sigma')$ to $\server$,
% who then verifies $e(\vk, \pp_{i+1}) \isequal e(\genone, \sigma')$ with $\vk = \pk_{1} + \ldots + \pk_{i+1}$.
% If the verification passes, $\server$ updates its state to $\pp \leftarrow \pp'$ and $\sigma \leftarrow \sigma'$ and stores $(\pk_{1}, \ldots, \pk_{i+1})$.


\paragraph*{Adding Operators and Contract into the Picture.}
The job of an operator $\server$ is to coordinate the contribution in a batch.
It collects the $\pk$s from the contributors and relay the latest $\pp$ and $\sigma$.
Once it has gathered enough contributions, it uploads to $\contract$ the final $\pp$ with an aggregated proof:
\begin{align*}
\pi_{\server} = \mathsf{agg}_{\mathsf{straw}}(\{\pi_{i} = (\sigma_{i}, \pk_{i})\}_{i \in [1..m]}) \defn (\sigma_{m}, \vk = \sum_{i \in [i..m]} \pk_{i})
\end{align*}
% , it uploads to $\contract$ the $\pp$ with $\pi_{\server} = (\sigma, \vk)$, where $\vk$ is the sum of all $\pk$s.

The contract $\contract$ will verify $\pp$ with $\pi_{\server}$ using \Cref{eqt:single-pairing-check} (and maintaining the fraud proof mechansim), and then update the $\pp$.
Then, another operator can take over by feteching the $\pp$ and $\sigma$ from $\contract$.

\paragraph*{Maintaining $\vk$ on $\contract$.}
Notice, an operator might not have access to the $\pk$s kept by other operators, and thus it cannot compute the $\vk$ by summing all $\pk$s.
Our strawman solution is to let $\contract$ store $\prevk$, a verification key for the previous update.
When a new operator comes with new $\{\pk_{i}\}_{i}$,
it submits $\curvk = \sum_{i} \pk_{i}$ to $\contract$, who then computes $\vk = \prevk + \curvk$.
Once the submission is verified, $\contract$ also udpates $\prevk \leftarrow \vk$
% it can compute the new $\vk' = \vk + \sum_{i} \pk_{i}$ on top of the piror $\vk$.
% \paragraph*{Submitting the Aggregated $\pp$ to the Contract}
% When $\server$ deems it has collected enough contributions from $m$ contributors,
% it can submit its latest $\pp$, $\sigma$, and $\vk = \pk_{1} + \ldots + \pk_{m}$ to the smart contract $\contract$,
% which then updates the PoT string to $\pp$ if they pass the check in \Cref{eqt:single-pairing-check}.
% % $e(\vk, \pp.Q_1) = e(\genone, \sigma)$.

% \lucien{Todo: combine the multi-$\server$ into this section}

% \pparagraph{Strawman Scheme: Extending Multi-$\user$ Approach}
% A straightforward approach is to extend our prIor multi-$\user$ aggregation protocol.
% Suppose the prior coordinator $\server$ additionally uploaded $\prevk$ and $\sigma$ on $\contract$ as the proof for $\checkone$.
% The new coordinator $\server'$ requires each contributor $\user_{i}$ (with $\pk_{i}$) to update $\sigma$ similar to \Cref{eqt:single-update}.

% After collecting enough updates, $\server'$ uploads to $\contract$ the new $\pp$ with the latest $\sigma$ and a new ``verification key'' $\curvk = \pk_{1} + \pk_{2} + \ldots$.
% Finally, $\contract$ accepts this update only if $\pp$, $\sigma$ and a new verification key $\vk = \prevk + \curvk$ can pass \Cref{eqt:single-pairing-check}.
% $\contract$ also updates $\prevk \leftarrow \vk$ for a valid update.

\subsubsection{Contribution Inclusion Check}
However, we are facing an issue for the inclusion check:
Seeing the $\pp$, $\sigma$, and $\vk$ on $\contract$,
a contributor $\user_{i}$ has no way to confirm that its contribution is indeed included.
$\server$ could pretend to accept the $\user_{i}$'s contribution, but then discard that contribution and develop an independent $\pp$.
The final $\pp$ and $\sigma$ will look different from $\user_{i}$'s $\pp$ and $\sigma$,
and thus $\user_{i}$ cannot verify whether its contribution is included in the $\pp$.

\pparagraph{Strawman Inclusion Check Scheme}
To make it clearer, we want a protocol to assure $\user_{i}$ with random value $r_{i}$ that $\pp.Q_{1} = (r_{i} \cdot \ldots ) \gentwo$
A naive solution is to let $\server$ publish a list of the public keys $\stkey = (\pk_{1}, \ldots, \pk_{m})$ and let any $\user_{i}$ confirm that
$\vk = \pk_{1} + ... + \pk_{m}$ and $\pk_{i} \in \st_{\pk}$.

The intuition is that since $\vk$ contains $\user_{i}$'s $\sk_{i}$,
the final $\sigma$ should contain $\user$'s $\sigma = (\sk_{i} + \ldots) (r_{i} \cdot \ldots) \gentwo$ to pass the pairing equality check.
Because $\user$'s $\sigma$ contains $r_{i}$ and because, again, the pairing equality check, $\pp.Q_{1}$ should also contains $r_{i}$.
More formally, we hope the following chain of reasoning holds
\begin{align*}
  e(\vk, \pp.Q_1) = e(\genone, \sigma) &\text{ and } \vk = \sk_{i} \genone + \ldots \\
  \implies\quad\quad e((\textcolor{red}{\sk_{i}} + \ldots) \genone, \pp.Q_1) &= e(\genone, (\textcolor{red}{ \sk_{i}} + \ldots) (\textcolor{red}{r_{i}} \cdot \ldots) \gentwo) \\
  \implies e((\sk_{i} + \ldots) \genone, (\textcolor{red}{r_{i}} \cdot \ldots) \gentwo) &= e(\genone, (\sk_{i} + \ldots) (r_{i} \cdot \ldots) \gentwo) \\
  \implies\quad\quad\quad\quad\quad\quad\quad\quad\quad \pp.Q_{1} &= (r_{i} \cdot \ldots)  \gentwo
\end{align*}
% To resolve this issue, we propose another protocol that allows

\pparagraph{(Intra-Coordinator) Rogue Key Attack}
However, this check scheme is insecure.
In BLS-style schemes, there exists a well-known attack called \emph{Rogue Key Attack}.

In the context of signatures,
an adversary can forge an aggregate signature on an arbitrary message that has never been signed by the victim.
In our context, a rogue key attack allows an adversary to falsely convince a contributor that its randomness is included in the latest $\pp$.

Here we demonstrate the attack in our context.
Suppose $\user$ with $\pk$ is the victim.
After receiving the $\pk$ from this contributor, a malicious $\server$ discards everything else.
Then, it proceeds with a compromised contributor $\user'$ with $(\sk'$, $\pk')$ and uploads the final $\pp$ that consists of only $\user'$'s contribution.
% , and $r' \in Z_p^{*}$
% In other words, $\pp.Q_{1} = r' \gentwo$.

The clever trick here is how to convince $\user$ its contribution is included.
$\server$ publishes $\stkey = (\pk, \pk' - \pk)$ and $\vk = \pk + (\pk' - \pk)  = \pk'$.
Notice, $\user$'s $\pk$ gets ``cancelled'' here.
$\server$ can just use $\sk'$ to compute a valid $\sigma = \sk' \cdot \pp.Q_{1}$
However, $\user$ could be convinced because $\pk \in \stkey$.

% At the first glance, it seems to be a failed attack because if the malicious $\server$ sets $\vk = \pk_{1} + \pk_{2}$,
% $\server$ cannot produce a $\sigma$ that passes the pairing equality check.
% Nevertheless,
% the malicious $\server$ can side-step this issue by including an artificial public key $-\pk_{1}$ in $\vk$.
% Now, $\vk = \pk_{1} + \pk_{2} - \pk_{1} = \pk_{2}$, and thus it can pass the verification with $\sigma = \sk_{2} r_{2} \gentwo$.
% Meanwhile, $\user_{1}$ might be convinced about the inclusion of its contribution because $\pk_{1} \in \st_{\pk} = \{ \pk_{1}, \pk_{2}, -\pk_{1} \}$

% An attempt to resolve this issue is let $\user_{3}$ to ensure that no $-\pk_{1}$ exists on the public key list.
% Still, an adversary can simply change the artificial key to $-\pk_{1} + \pk_{3}$ with a known $\sk_{3}$ to evade this detection.

\pparagraph{Proof-of-Possession (PoP)}
To defend against this attack, we adopt the proof-of-possession approach~\cite{proof-of-possion-bls}, which requires each public key owner to sign on a hash value of its public key using the secret key.
Each $\user$ now also needs to provide $\pos = \sk \cdot \hashgp(\pk)$ to $\server$.
A $\pos$ can be verified by $e(\pk, \hashgp(\pk)) =_{?} e(\genone, \pos)$.
The idea is that an adversary who generates artificial keys ($\pk' - \pk$ in our example) does not know the corresponding secret keys ($\sk' - \sk$),
so it cannot sign on the hash value.
% For example, this approach defeats the above attack:
% % Take the above attack as an example,
% for $\pk_{3} = -\pk_{1}$,
% a malicious $\server$ does not know $-sk_{1}$ so it cannot produce the $\pos = -\sk_{1} \hashgp(-\pk_{1})$.

\pparagraph{Our Final Inclusion Check Protocol}
Now, we upgrade our inclusion check protocol.
To show the proof of posession of all $\pk$s that constitute $\vk$,
$\server$ lists all pairs of $\stkey = \{(\pk_{i}, \pos_{i})\}_{i}$ on its public server.
During verification, $\user_{j}$ with $\pk_{j}$ confirms:
i) $(\pk_{j}, *) \in \stkey$;
% ii) $\vk = \pk_{1} + \ldots + \pk_{m}$;
ii) $\curvk = \sum_{i} \pk_{i}$;
and iii) the validity of all $\pos$s.

With the PoP check in place, our scheme is secure for the inclusion check, and we formally prove its security in \cref{thm:incl-snd}.


\subsubsection{Progressive Key Aggregation}
Nevertheless,
% this above defense only partially solve the problem. The protocol still suffers from a variation of rogue key attacks.
% Note
the proof of possession approach can prevent \emph{intra-coordinator} rogue key attacks,
where the rogue keys exist among a coordinator's collected $\pk$s.
However, it does not eliminate the \emph{inter-coordinator} rogue key attacks, where the rogue keys come from other coordinators.

% \todo{this is too long/detailed. reviewers may get lost.}
% Now, we introduce how to further upgrade our protocol to support multiple $\server$s to update the $\pp$ on a smart contract $\contract$ sequentially.

% The high-level procedures are as follows: After a coordinator $\server$ uploads $\pp$ and the proofs on-chain,
% another coordinator $\server'$ reads $\pp$ and the proofs from (the transaction history of) $\contract$, and uploads $\pp'$ with proof to $\contract$.
% Importantly, the proof should assure $\contract$ that $\server'$ knows the added randomness.

\pparagraph{(Inter-Coordinator) Rogue Key Attacks}
Here, we illustrate this attack.
Suppose the (honest) first coordinator $\server_{1}$
% has only one contributor with public key $\pk_{1}$ and
has uploaded $\pp$ and $\vk_{1}$ with its proof.
Now, $\prevk = \vk_{1}$.
A malicious second coordinator $\server_{2}$ with $(\sk_{2}, \pk_{2})$ can then perform a ``key cancellation'' to remove $\vk_{1}$ from the next verification key
% and gain complete control of the secret keys in $\vk_2$.
% This involves
% $\server_2$ generating a secret-public key pair $(\sk_{2}, \pk_{2})$ and setting
It simply uploads $\curvk = -\vk_{1} + \pk_{2}$.
Notice, the new verification key to check $\server_{2}$'s update becomes
\begin{align*}
    \vk = \prevk + \curvk = \vk_{1} + (-\vk_{1} + \pk_{2}) = \pk_{2}.
\end{align*}
Now, $\server_{2}$ can use its $\sk_{2}$ to produce a valid $\sigma$ on arbitrary $\pp$.
% without building on top of the previous $\pp$.

\pparagraph{Unhelpful PoP}
Unfortunately, the PoP approach, which defended against the intra-coordinator rouge key attack, does not work here.
It is too expensive for $\contract$ to verify all $\pk$s and $\pos$s, whose total size is linear to the number of contributions,
% To verify all $\pos$s of the new $\vk$,
% $\contract$ needs to read input data that contains all $\pk$s and $\pos$s, whose size is linear to the number of contributions.
% Furthermore, each verification on a $\pos$ require at least one \var{ECMULT}, which is an expensive on-chain operation.
% Either of these issues already
defeating the purpose of a constant-size aggregate proof.

\pparagraph{Random Coefficients for $\vk$s and $\sigma$s}
To defend this attack, we resort to a ``random coefficient'' approach~\cite{ctrsa/FerraraGHP09,eurocrypt/CamenischHP07,asiacrypt/BonehDN18},
which is a recurring technique for batched siganture verification.
Instead of computing $\vk = \prevk + \curvk$,
$\contract$ now samples two random coefficients $\rho_{1}, \rho_{2} \sample \Zp^{*}$
and computes $\vk = \rho_{1} \prevk + \rho_{2} \curvk$.
% Now, the malicious $S_{2}$ cannot cancel out the prior verification key
Now, the key cancellation trick cannot help a malicious $\server$ to get rid of the prior $\prevk$
because with overwhelming probability
\begin{align*}
  \vk &= \rho_{1} \prevk + \rho_{2} \curvk = \rho_{1} \vk_{1} + \rho_{2} (-\vk_{1} + \pk_{2})
  \\&= (\rho_{1} - \rho_{2}) \vk_{1} + \ldots \text{ and } (\rho_{1} - \rho_{2}) \neq 0
\end{align*}

% Similarly, $\sigma$ also needs
Obviously, $\sigma$ computed by our prior approach cannot pass \Cref{eqt:single-pairing-check}
as $\vk$ is no longer a simple sum of all $\pk$s.
To cater for the randomly combined $\vk$s, the coordinator and contributors need to instead update two $\sigma$s: $\presig$ and $\cursig$.
% $\presig$ and $\cursig$ should be able to pass the verificaiotn with $\prevk$ and $\curvk$, respectively.
In our protocol, a $\server$ fetches $\presig$ from $\contract$ and then ask a $\user$ with a random value $r$, new $\pp$, and key pair $(\sk, \pk)$ to update as following
\begin{align*}
  \presig \leftarrow r \cdot \presig \quad \cursig \leftarrow \sk \cdot \pp.Q_{1} + r \cdot \cursig
\end{align*}
Notice, $\presig$ and $\cursig$ are supposed to contain the $\sk$s in $\prevk$ and $\curvk$, respectively.

Then, $\user$ sends $\pp, \pi = (\presig, \cursig, \pk, \pos)$ to $\server$.
After gathering all the updates from contributors, 
$\server$  uploads to $\contract$ the final $\pp$ and 
% $\pi_{\server} = (\presig$, $\cursig, \curvk)$.
\begin{align*}
\pi_{\server} = \mathsf{agg}(\{\pi_i\}_{i \in [m]}) \defn (\pi_m.\presig, \pi_m.\cursig, \curvk = \sum_{i \in [m]} \pk_i)
\end{align*}
% $\curvk = \pk_{1} + \ldots + \pk_{m}$, where $\pk_{1}, \ldots, \pk_{m}$ are the $\pk$s of $\server$'s contributors.
% , while $\cursig$ contains the $\sk$s in $\curvk$, \ie, those from the current $\server$'s contributor.
% Notice, $\presig$ contains the $\sk$s in $\prevk$, which are from the previous contributors, while $\cursig$ contains the $\sk$s in $\curvk$, \ie, those from the current $\server$'s contributor.


Finally,
$\contract$ computes $\vk = \rho_{1} \prevk + \rho_{2} \curvk$ and $\sigma = \rho_{1} \presig + \rho_{2} \cursig$ and
uses \Cref{eqt:single-pairing-check} to verify them.
% verifies
% \begin{align*}
%   e(\vk, \pp.Q_{1}) \isequal e(\genone, \sigma)
% \end{align*}
The correctness and soundness holds because the above verification is (almost) equivalent to verifying
\begin{align*}
e(\prevk, \pp.Q_{1}) \isequal e(\genone, \presig)
  \wedge
e(\curvk, \pp.Q_{1}) \isequal e(\genone, \cursig)
\end{align*}
and for each of these equality checks, we can apply our prior conclusion about the security properties.
% about the consistency of $\pp.Q_{1}$, $\sigma$, and $\vk$.



\pparagraph{Progressive Key Aggregation}
The random combination on $\sigma$ and $\vk$ is \emph{not} only for this one-time verification.
After passing the verification, $\contract$ will update in its state:
\begin{align*}
  \prevk \leftarrow \rho_{1} \prevk + \rho_{2} \curvk \quad
  \presig \leftarrow \rho_{1} \presig + \rho_{2} \cursig
\end{align*}
Without these random coefficients in the update $\prevk$, an inter-coordinator rogue key attack is still possible.

Another issue for $\contract$ is how to sample $\rho_{1, 2}$.
In practice, $\contract$ is implemented on a blockchain and $\contract$'s randomness can be biased to favor the adversary.
Here, we propose $\contract$ samples $\rho_{\{1,2\}}$ via the following hashing
\begin{align*}
\rho_{j} = H(\prevk ||\curvk || \presig || \cursig || \pp.Q_{1} || j ) \text{ for } j \in \{1, 2\}
\end{align*}

We provide a formal security analysis and proofs
% this progressive key aggregation (on random coefficients)
against inter-coordinator rogue key attacks in Theorem~\ref{thm:incl-snd} (Lemma~\ref{lem:hash-zippel} and Lemma~\ref{lem:snd-after-t}).


%%% Local Variables:
%%% mode: LaTeX
%%% TeX-master: "main"
%%% End:


==> prf-log-ag.tex <==
  \begin{proof}
    By inspecting~\Cref{fig:prf-coeff-sk}.
    \begin{figure*}[!t]
    {\small
      \fbox{ \parbox{0.975\textwidth}{
          \begin{align*}
            \!\text{For $G \in \gpone$}: \\
            G &=
                \overbrace{\coeff{G}{\pk} }^{A_{G}} \cdot \pk
                + \overbrace{ \sum_{i \in [1..t-1]} \coeff{G}{\vk_{i}} \vk_{i}
                + \sum_{i=[1..t-1], j} \coeff{G}{\pk_{i, j}} \cdot \pk_{i, j}
                + \sum_{i=[1..t-1], j \in [1..n]} \coeff{G}{\tau_{i}^{j}} \cdot \tau_{i}^{j} \cdot \genone
                + \coeff{\vk^{*}}{1} \cdot \genone}^{\mathcal{B}_{G}} \\
            \log G &= A_{G} \cdot \sk + \log \mathcal{B}_{G} \\
            \!\text{For $G \in \gptwo$}: \\
            G &=
                \coeff{G}{\pos} \cdot \pos +\coeff{G}{\cursig'} \cdot \cursig' + \mathcal{B}_{G} \\
            % &=
    %             \coeff{G}{\presig'} \cdot \presig' + \coeff{G}{\cursig'} \cdot \cursig' + \coeff{G}{\pos} \cdot \pos
    %           + \sum_{i=[1..t-1], j} \coeff{G}{\pos_{i,j}} \cdot \pos_{i,j}
    %           + \sum_{i=[1..t-1]} \coeff{G}{{\presig}_{i}} \cdot {\presig}_{i}
    %             \\&+ \sum_{i=[1..t]} \coeff{G}{{\cursig}_{i}} \cdot {\cursig}_{i}
    %           + \sum_{i=[1..t], j \in [1..k]} \coeff{G}{\tau_{i}^{j}} \cdot \tau_{i}^{j} \cdot \gentwo
    %             \coeff{G}{\presig'} \cdot \presig' + \coeff{G}{\cursig'} \cdot \cursig' + \coeff{G}{\pos} \cdot \pos \\
    % &+ \sum_{i=[1..t], j} \coeff{G}{\pos_{i,j}} \cdot \pos_{i,j} \\
    % &+ \sum_{i=[1..t]} \coeff{G}{{\presig}_{i}} \cdot {\presig}_{i}
    %  + \sum_{i=[1..t]} \coeff{G}{{\cursig}_{i}} \cdot {\cursig}_{i} \\
    % &+ \sum_{i=[1..t], j \in [1..k]} \coeff{G}{\tau_{i}^{j}} \cdot \tau_{i}^{j} \cdot \gentwo \\
    %       \log \presig^{*}
    % &= \coeff{\presig^{*}}{\presig'}
    %   \cdot (\delta_{\mathsf{pre}}) \cdot (r \cdot \xi \cdot \tau_{i-1}) \\
    %   &+ \coeff{\presig^{*}}{\cursig'}
    %   \cdot (\sk + \delta_{\mathsf{cur}}) \cdot (r \cdot \xi \cdot \tau_{i-1}) \\
    %   &+ \coeff{\presig^{*}}{\pos} \cdot \sk \cdot \log H(\pk) \\
    % &+ \sum_{i=[1..t], j} \coeff{\presig^{*}}{\pos_{i,j}} \cdot \log \pos_{i,j} \\
    % &+ \sum_{i=[1..t]} \coeff{\presig^{*}}{{\presig}_{i}} \cdot \log {\presig}_{i}
    %  + \sum_{i=[1..t]} \coeff{\presig^{*}}{{\cursig}_{i}} \cdot \log {\cursig}_{i} \\
    % &+ \sum_{i=[1..t], j \in [1..k]} \coeff{\presig^{*}}{\tau_{i}^{j}} \cdot \tau_{i}^{j} \\
    % &= (\coeff{\presig^{*}}{\cursig'} \cdot (r \cdot \xi \cdot \tau_{i-1}) +
    %   \coeff{\presig^{*}}{\pos} \cdot \log H(\pk)) \cdot \sk + B_{\presig^{*}}(\tau_{t-1}) \\
    % \log Q_{1}^{*} &= w
          % \end{align*}
          % \vspace{-30pt}
          % \begin{align*}
            \mathcal{B}_{G} &=
               % \underbrace{
            \coeff{G}{\presig'} \cdot \presig'
            + \sum_{i\in[1..t-1], j} \coeff{G}{\pos_{i,j}} \cdot \pos_{i,j}
              + \sum_{i\in[1..t-1]} \coeff{G}{{\presig}_{i}} \cdot {\presig}_{i}
                \\&+ \sum_{i\in[1..t-1]} \coeff{G}{{\cursig}_{i}} \cdot {\cursig}_{i}
              + \sum_{i\in[1..t-1], j \in [1..k]} \coeff{G}{\tau_{i}^{j}} \cdot \tau_{i}^{j} \cdot \gentwo \\
               % }_{\mathcal{B}_{G}}
          % \end{align*}
          %   \vspace{-10pt}
          % \begin{align*}
            \log G &=
                     \underbrace{
                     (\coeff{G}{\cursig'} \cdot r \cdot \xi + \coeff{G}{\pos} \cdot \log H(\pk))}_{A_{G}} \cdot \sk +
            \underbrace{r + \log \cursig + \log \mathcal{B}_{G}}_{B_{G}}
          \end{align*}
        Note: $\pos = \sk \cdot \log H(\pk)$ and $\log \cursig' = \sk \cdot r \cdot \xi + r \cursig$.
        } } }
      \caption{The Proof of Lemma~\ref{lem:coeff-sk}. We prove it by expressing $G$ as a linear combination of all group elements $\advinclude$ have seen. For $G \in \gpone$, $\pk$ (with $\log \pk = \sk$) is the only group elements related to $\sk$ in $\gpone$.
        For $G \in \gptwo$, $\cursig'$ and $\pos$ are the only elements relevent to $\sk$.
        The exact composition of $B_{G}$ does not matter for our proof. We list them here to ensure ourselves not missing any group elements by exhaustion.}
    \label{fig:prf-coeff-sk}
    \end{figure*}
  \end{proof}

